Diffusion Model as Representation Learner

Diffusion Probabilistic Models (DPMs) have recently demonstrated impressive results on various generative tasks.Despite its promises, the learned representations of pre-trained DPMs, however, have not been fully understood. In this paper, we conduct an in-depth investigation of the representation power of DPMs, and propose a novel knowledge transfer method that leverages the knowledge acquired by generative DPMs for recognition tasks. Our study begins by examining the feature space of DPMs, revealing that DPMs are inherently denoising autoencoders that balance the representation learning with regularizing model capacity. To this end, we introduce a novel knowledge transfer paradigm named RepFusion. Our paradigm extracts representations at different time steps from off-the-shelf DPMs and dynamically employs them as supervision for student networks, in which the optimal time is determined through reinforcement learning. We evaluate our approach on several image classification, semantic segmentation, and landmark detection benchmarks, and demonstrate that it outperforms state-of-the-art methods. Our results uncover the potential of DPMs as a powerful tool for representation learning and provide insights into the usefulness of generative models beyond sample generation. The code is available at \url{https://github.com/Adamdad/Repfusion}.

==> section/sup.tex <==
% \begin{align}
%     \mathcal{L}(D, E) &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||\bm\epsilon - VW(\mathbf{x} + \bm\epsilon)||^2_2]\\
%      &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||(\bm\epsilon - VW\bm\epsilon) - VW\mathbf{x}||^2_2]\\
%     &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||\bm\epsilon - VW\bm\epsilon||_2^2 + ||VW\mathbf{x}||^2_2] \\&(\text{$\bm\epsilon$ is independent of $\mathbf{x}$})\\
%      &= \mathbb{E}_{\bm\epsilon }[ ||(I - VW)\bm\epsilon||_2^2] +\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}||^2_2]\\
%       &= ||I- VW||^2_2\mathbb{E}_{\bm\epsilon }[ || \bm\epsilon||_2^2] +\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}||^2_2]\\
%       &= \sigma^2||I- VW||^2_2+\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}||^2_2]\\
% \end{align}

% \begin{align*}
%     \mathcal{L}(V, W) &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||\bm\epsilon - VW(\mathbf{x}_t)||^2_2]\\
%     &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||\bm\epsilon - VW(\sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t} \bm{\epsilon})||^2_2]\\
%      &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||(\bm\epsilon - \sqrt{1-\bar{\alpha}_t}VW\bm\epsilon) - \sqrt{\bar{\alpha}_t}VW\mathbf{x}||^2_2]\\
%     &= \mathbb{E}_{\mathbf{x}, \bm\epsilon }[ ||\bm\epsilon - \sqrt{1-\bar{\alpha}_t}VW\bm\epsilon||_2^2 + ||\sqrt{\bar{\alpha}_t}VW\mathbf{x}||^2_2] \\&(\text{$\bm\epsilon$ is independent of $\mathbf{x}$})\\
%      &= \mathbb{E}_{\bm\epsilon }[ ||(I - \sqrt{1-\bar{\alpha}_t}VW)\bm\epsilon||_2^2] + \bar{\alpha}_t\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}_0||^2_2]\\
%       &= ||I- \sqrt{1-\bar{\alpha}_t}VW||^2_2\mathbb{E}_{\bm\epsilon }[ || \bm\epsilon||_2^2] +\bar{\alpha}_t\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}_0||^2_2]\\
%       &=||I- \sqrt{1-\bar{\alpha}_t}VW||^2_2+\bar{\alpha}_t\mathbb{E}_{\mathbf{x}}[||VW\mathbf{x}_0||^2_2]\\
% \end{align*}

\section{Derivation for Linear AE Diffusion}
As stated in the paper, we consider an oversimplified case with linear autoencoder and skip connection that imitates the architecture of Unet~\cite{ronneberger2015u} used in DPMs. We assume $W_E\in \mathbb{R}^{d\times L}$, $W_D\in \mathbb{R}^{L\times d}$ and $W_S\in \mathbb{R}^{L\times L}$ are the encoding, decoding and skip-connection matrices. At time-step $t$, the encoder maps the input signal $\mathbf{x}_t = \sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t} \bm{\epsilon}$  to a hidden space $\mathbf{h}=W_E\mathbf{x}_t$, and the decoder maps it back to make the noise prediction $\hat{\bm \epsilon}=W_D\mathbf{h}+W_S \mathbf{x}_t$.
\begin{align*}
       \mathcal{L}(W_E,W_D, W_S) &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ ||\bm\epsilon - (W_DW_E\mathbf{x}_t + W_S\mathbf{x}_t)||^2_2]\\
       &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ ||\bm\epsilon - (W_DW_E + W_S) \mathbf{x}_t||^2_2]\\
       &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ ||\bm\epsilon - (W_DW_E + W_S) (\sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t} \bm{\epsilon})||^2_2]\\
       &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ ||\big(\bm\epsilon - (W_DW_E + W_S) \sqrt{1-\bar{\alpha}_t} \bm{\epsilon} \big)- \sqrt{\bar{\alpha}_t}(W_DW_E + W_S) \mathbf{x}_0||^2_2]\\
        &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ ||\bm\epsilon - (W_DW_E + W_S) \sqrt{1-\bar{\alpha}_t} \bm{\epsilon}||^2_2+||\sqrt{\bar{\alpha}_t}(W_DW_E + W_S) \mathbf{x}_0||^2_2]\quad \Big(\text{$\bm\epsilon$ is independent of $\mathbf{x}_0$}\Big)\\
        &= \mathbb{E}_{\mathbf{x}_0, \bm\epsilon }[ || \Big(I - \sqrt{1-\bar{\alpha}_t}(W_DW_E + W_S) \Big) \bm{\epsilon}||^2_2]+ \bar{\alpha}_t\mathbb{E}_{\mathbf{x}_0}[||(W_DW_E + W_S) \mathbf{x}_0||^2_2]\\
         &= ||I - \sqrt{1-\bar{\alpha}_t}(W_DW_E + W_S)||^2_2+\bar{\alpha}_t\mathbb{E}_{\mathbf{x}_0}[||(W_DW_E + W_S) \mathbf{x}_0||^2_2] \quad \Big(\text{$\bm{\epsilon}\sim \mathcal{N}(0,1)$ so that $\text{Cov}(\bm{\epsilon},\bm{\epsilon})=I$}\Big)\\
         &= ||I - \sqrt{1-\bar{\alpha}_t}(W_DW_E + W_S)||^2_2+\bar{\alpha}_t (W_DW_E + W_S)^\top \mathbb{E}_{\mathbf{x}_0}[|| \mathbf{x}_0||^2_2](W_DW_E + W_S) \\
         & \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad
         \Big(\text{Assume $\mathbb{E}[\mathbf{x}_0]=\mathbf{0}$ such that $\text{Cov}(\mathbf{x}_0,\mathbf{x}_0)=\mathbb{E}_{\mathbf{x}_0}[|| \mathbf{x}_0||^2_2]$ }\Big)\\
         &= ||I - \sqrt{1-\bar{\alpha}_t}(W_DW_E + W_S)||^2_2+\bar{\alpha}_t (W_DW_E + W_S)^\top \text{Cov}(\mathbf{x}_0,\mathbf{x}_0) (W_DW_E + W_S) 
\end{align*}
If we assume $P =W_DW_E + W_S$, and $\text{Cov}(\mathbf{x}_0,\mathbf{x}_0)=\Sigma_{xx}$, we gets to the formulation in the paper
\begin{align}
    \mathcal{L}(W_E,W_D, W_S) = \underbrace{\bar{\alpha}_t P^\top \Sigma_{xx} P }_{\text{Representation Learning}}+\underbrace{||I - \sqrt{1-\bar{\alpha}_t}P||^2_2}_{\text{Regularization}}\label{eq:1}
\end{align}
As stated in the paper, this formulation indicates that there exists a trade-off between acquiring a meaningful representation and penalizing the optimal parameter spectrum. 

\section{Pseudo-code for \name}
Algorithm~\ref{alg:pseudo} presents the pseudo-code for our proposed \name~to harvesting the knowdege from pretrain DPMs. 

In the first stage of our methodology, we distill the representation of a pre-trained DPM, denoted by $\bm s(\cdot, \cdot; \bm\theta^*)$, into a student encoder $f(\cdot; \bm \theta_{f})$. The objective of this stage is to transfer knowledge from the pre-trained DPM to the student encoder, thereby enabling the encoding of input data into a meaningful latent space.

To determine the optimal distillation timestep, we employ a policy network denoted by $\bm \pi_{\bm \theta_\pi}(t|\mathbf{x})$ within a reinforcement learning setting. Specifically, we utilize the REINFORCED algorithm to optimize the policy network to maximize the predictivity of the extracted feature. This approach allows the student encoder to capture task-relevant information during distillation, leading to improved performance.

During the second stage, we employ standard backpropagation to fine-tune the student decoder on the desired dataset with full annotations.

\begin{algorithm}[H]
\small
	\caption{Repfussion} 
		\label{alg:pseudo}
	\begin{algorithmic}[1]
	\State \textcolor{SeaGreen}{\# Distill from Trained DPM}
		\For {$\text{epoch}=1,2,\ldots,\text{max\_epoch}$}
    		% \State Initialize the network partition $\{B_{i}^{(k)}\}_{k=1}^K|_{0}$ and clustering $A|_0$
			\For {$t=1,2,\ldots, T$}
				\State Predict the timestep $t$ by sampling from the action distribution $t\sim \text{Categorical}_T(\bm\pi_{\bm\theta_\pi}(t|\mathbf{x}))$.
				\State Extract the features according to the timestep $\mathbf{z}^{(t)}\leftarrow \bm s(\mathbf{x}, t; \bm\theta^*)$ and $\mathbf{z} \leftarrow f(\mathbf{x}; \bm\theta_f)$.
                \State Update the student to minimize distillation loss, $\bm\theta_f \leftarrow \bm\theta_f - \nabla_{\bm\theta_f}\mathbb{E}[\mathcal{L}_{\text{kd}}(\mathbf{z}^{(t)},\mathbf{z})]$.
				\State Update additional decoder $g$ to minimize task loss, $\bm\theta_g \leftarrow \bm\theta_g - \mathcal{L}_{\text{task}}(g(\mathbf{z}^{(t)}), y)$.
                \State Update the policy network $\bm \pi$ to maximize the reward, $\bm\theta_{\bm \pi} \leftarrow \bm\theta_{\bm \pi} + J(\bm\theta_{\bm \pi})$. 
			\EndFor
		\EndFor
		\State \textcolor{SeaGreen}{\# Finetune on Task Label}
		\For {$\text{epoch}=1,2,\ldots,\text{max\_epoch}$}
		    \State Update the student to minimize the task loss, $\bm\theta_{f} = \bm\theta_{f} - \nabla_{\bm\theta_{f}}\mathbb{E}[\mathcal{L}_{\text{task}}(y,\hat{y})]$,where $\hat{y} = f(\mathbf{x};\bm\theta_f)$.
		\EndFor  
	\end{algorithmic} 

\end{algorithm}

\section{Additional Experiment}
This section presents additional experiments that serve to reinforce the underlying motivation and validate the effectiveness of our \name~models.
\subsection{What Timestep has Been Selected?}
In the main paper, we describe our significant contribution of automating representation extraction through adaptive time step selection. This is achieved by employing a reinforced strategy. However, a critical question arises: "Which action will our algorithm prefer, and ultimately converge upon?" This section aims to address this issue by examining the time selection outcomes of our proposed scheme on the CIFAR-10 dataset.

Figure~\ref{fig:cifar-timestep} illustrates the average timestep selected in each training batch, with the standard deviation presented as a shadow around the mean value. It is clear from the graph that, starting from a more near uniform selection, the policy network $\bm\pi$ gradually converges to a small time index of approximately 100. This outcome is in line with our derivation in Section 3 of the main paper, where we demonstrated that a small timestep leads to optimal performance for recognition task distillation.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\linewidth]{iccv2023AuthorKit/fig/timestepselect.pdf}
    \caption{Average Time step selected by \name~at different training iterations on CIFAR-10.}
    \label{fig:cifar-timestep}
\end{figure}


% \subsection{ImageNet Classification}
% We further extend our framework to tackle large-scale image classification using ImageNet datasets~\cite{deng2009imagenet} datasets. Following the same pipeline, we first distill a ResNet-18 network from a well-trained DDPM\footnote{\url{https://openaipublic.blob.core.windows.net/diffusion/jul-2021/256x256_diffusion_uncond.pt}}. Due to the large computational complexity of diffusion model, we only distilled the student for 10 epochs with a batch size of 96, employing the AdamW optimizer with an initial learning rate of 2.5e-4 and cosine learning rate decay. After distillation, we proceeded to fine-tune the student network on the ImageNet dataset using a typical protocol. This involved training the network for 100 epochs, with an initial learning rate of 0.1 and step learning rate decay at the 30th and 60th epochs.

% Table~\ref{tab:imagenet} presents the top1 and top5 accuracy achieved by our proposed method on the ImageNet validation set. To provide context, we also compare the results with two classical knowledge distillation techniques, namely output logits matching (KD)\cite{Hinton2015DistillingTK} and attention transfer (AT)\cite{zagoruyko2016paying}. We observe that \name, despite being based on a short time of knowledge distillation, achieves the best results.

% Our success can be attributed to the powerful representation of the well-trained DDPM model that we leveraged. By incorporating this representation into the distillation process, we were able to produce a highly accurate ResNet-18 network that could perform well even in the most complex and computationally demanding tasks.

% \begin{table}[H]
%     \centering
%       \vspace{-5mm}
%         \caption{Test accuracy on ImageNet.}
%     \label{tab:imagenet}
%     \vspace{-3mm}
%     \begin{tabular}{l|l|l}
%     \hline
%         Method & Top-1 & Top-5 \\
%         \hline
%         ResNet-18 & 69.90 & 89.43\\
%         + KD (ResNet-34) & 70.66 &90.00\\
%          + AT (ResNet-34) & 70.90 &90.63\\
%          \hline
%         + \name & \textbf{71.25}(\textcolor{Green}{+1.35}) & \textbf{91.33}(\textcolor{Green}{+1.90}) \\\hline
%     \end{tabular}

% \end{table}

\subsection{Results Visualization}
Our numerical experiment strongly suggests that \nameis particularly efficient for dense prediction tasks, such as image segmentation and landmark detection. To further corroborate this observation, we provide supplementary visual results in Figure\ref{fig:keypointmore} and Figure~\ref{fig:segmore}.

Figure~\ref{fig:keypointmore} illustrates the results obtained using a top-down simple head in combination with the ResNet-50 backbone. We present visualizations of the detected keypoints on several testing subsets, including \texttt{largepose}, \texttt{makeup}, and \texttt{occlusion}. Our approach exhibits robust and accurate detection results even under challenging conditions, such as low-quality images, complex facial expressions, and varying poses and visibility.
\begin{figure}[H]
    \centering
    \vspace{-3mm}
      \begin{subfigure}[b]{\linewidth}
         \centering
    \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/facelandmark_pose.pdf}\vspace{-1mm}
        \caption{Results on \texttt{largepose} subset.}
         \label{fig:largepose}
     \end{subfigure}
       \begin{subfigure}[b]{\linewidth}
         \centering
\includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/facelandmark_makeup.pdf}\vspace{-1mm}
         \caption{Results on \texttt{makeup} subset.}
         \label{fig:makeup}
     \end{subfigure}
            \begin{subfigure}[b]{\linewidth}
         \centering
\includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/facelandmark_occ.pdf}\vspace{-1mm}
         \caption{Results on \texttt{occlusion} subset.}
         \label{fig:makeup}
     \end{subfigure}
    \caption{Landmark detection on n WFLW dataset with \name~and ResNet-50.}
    \label{fig:keypointmore}
\end{figure}

In Figure~\ref{fig:segmore}, we present the semantic masks generated by the BiSeNetv1 model utilizing the ResNet-50 backbone, distilled and trained exclusively on CelebAMask-HQ. We note that the model's robustness is demonstrated by its excellent performance even when subjected to cross-dataset evaluations, despite the medium domain gap. This finding suggests that the proposed approach holds promise for achieving strong performance in challenging segmentation tasks.
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/celebamask.pdf}
        \caption{Results on CelebAMask-HQ.}
         \label{fig:largepose}
     \end{subfigure}
       \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/celeba.pdf}
        \caption{Inference Results on CelebA.}
         \label{fig:largepose}
     \end{subfigure}
            \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/fig/ffhq.pdf}
        \caption{Inference Results on FFHQ.}
         \label{fig:largepose}
     \end{subfigure}
    \caption{Face Parsing results visualization on CelebAMask-HQ, CelebA with \name~distilled BiSENet ResNet-50 trained on CelebAMask-HQ only.}
    \label{fig:segmore}
\end{figure}
% \subsection{Face Attribute Multi-label Classification}
% the per-class metrics (average per-cass precision (CP), recall (CR), F1-score (CF1)) and 2) the overall metrics (the average overall precision (OP), recall (OR), F1-score (OF1))

% \begin{table}[H]
%     \centering
%     \caption{Performance on CelebA face attribute multi-label classification.}
%     \label{tab:my_label}
%     \begin{tabular}{l|c|c|c|c|c|c|c}
%     \hline
%         Method & mAP & CP &CR &CF1 & OP &OR &OF1 \\
%         \hline
%         ResNet-18 & 66.55&63.29&5.32&9.81&99.77& 9.86&17.94\\ 
%         + \name &\\
%         \hline
%         ResNet-50 & \\ 
%         + \name &\\
%         \hline
%     \end{tabular}
    
% \end{table}
% \subsection{Face Detection}

% \subsection{Church Classification and Detection}





\section{Experimental Details}
\subsection{Baselines}
\noindent\textbf{Self-supervised Pre-training.} To train the ResNet-50 on the CelebA-HQ dataset, we utilized the official implementations of MoCov2\footnote{\url{https://github.com/facebookresearch/moco}}, SwAV, and DeepClusterv2\footnote{\url{https://github.com/facebookresearch/swav}}. Since these methods are self-supervised, they do not leverage the segmentation labels. We keep all hyper-parameters the same as the original paper, to make sure the comparison is indeed fair.

\noindent\textbf{Representation Learned From GANs.} Several attempts have been made to utilize the latent space of GANs for representation learning, such as BigBiGAN~\cite{donahue2019large} and GH-Feat~\cite{xu2021generative}. However, it should be noted that these approaches are implemented using TensorFlow, and the pre-trained weights are based on different datasets. Therefore, in this work, we do not conduct a direct comparison between \name~and these methods. We acknowledge that this presents a technical challenge, but we plan to address this limitation in the near future.
\subsection{Semantic Segmentation}
In this study, we validated the segmentation performance of \nameusing the CelebAMask-HQ dataset\cite{CelebAMask-HQ}. The dataset consists of 30,000 high-resolution facial images, each accompanied by a segmentation mask containing 19 facial attributes listed in Table\ref{tab:CelebAMask-HQ_cat}. We randomly partitioned the dataset into 24,183 samples for training, 2,993 for validation, and 2,824 for testing. Initially, we distilled ResNet-18 and ResNet-50 on the CelebAMask-HQ dataset for 200 epochs. Subsequently, the distilled model was used as the feature extractor in BiSeNetv1 and fine-tuned for face parsing. The hyperparameters used during the distillation process are presented in Table~\ref{tab:distill_hyper}, while those for fine-tuning can be found in Table~\ref{tab:finetune_hyper}. Table~\ref{tab:featurematchs} provides the names of the distillation feature pairs. The model was implemented using \texttt{mmseg}\footnote{\url{https://github.com/open-mmlab/mmsegmentation}}.

\begin{table}[H]
    \centering
        \caption{Category Names for CelebAMask-HQ.}
    \label{tab:CelebAMask-HQ_cat}
\begin{tabular}{l|l|l|l|l}
\hline
\multicolumn{5}{c}{Label list} \\\hline
0: 'background'                & 1: 'skin'            & 2: 'nose'            & 3: 'eye\_g' & 4: 'l\_eye' \\
5: 'r\_eye'                    & 6: 'l\_brow'         & 7: 'r\_brow'         & 8: 'l\_ear' & 9: 'r\_ear' \\
10: 'mouth'                    & 11: 'u\_lip'         & 12: 'l\_lip'         & 13: 'hair'  & 14: 'hat'   \\
15: 'ear\_r'                   & 16: 'neck\_l'        & 17: 'neck'           & 18: 'cloth' &             \\\hline
                          
\end{tabular}
\end{table}

\begin{table}[t]
    \centering
        \caption{Distillation Phase Hyper-parameter Setting on Various Datasets.}
    \label{tab:distill_hyper}
    \begin{tabular}{l|c|c|c}
    \hline
        \textbf{Dataset} & \textbf{CIFAR-10} &  \textbf{TinyImageNet} & \textbf{CelebAMask-HQ}  \\\hline
        Teacher link & \texttt{ddpm-cifar10-32}\tablefootnote{\url{https://huggingface.co/google/ddpm-cifar10-32} } &\texttt{64x64\_diffusion}\tablefootnote{\url{https://openaipublic.blob.core.windows.net/diffusion/jul-2021/64x64_diffusion.pt} } & \texttt{
ddpm-ema-celebahq-256}\tablefootnote{\url{https://huggingface.co/google/ddpm-ema-celebahq-256}}\\\hline
        Optimizer & SGD & SGD & SGD \\\hline
        lr & 0.1 & 0.1 & 0.1 \\\hline
        momentum & 0.9 & 0.9 & 0.9 \\\hline
        bs & 128 & 64 & 64 \\\hline
        EMA momentum & 0.999 & 0.999 & 0.999  \\\hline
        weight decay & 1e-4 & 1e-4 & 1e-4\\\hline
        distillation weight & 1/1000/1 & 1/1000/1 & 1\\\hline
        distillation loss & Hint/AT/RKD & Hint/AT/RKD & Hint\\\hline
        training time &  200 epoch  &200 epoch &200 epoch  \\ \hline
    \end{tabular}

\end{table}
\begin{table}[t]
\small
    \centering
        \caption{Finetuning Phase Hyper-parameter Setting on Various Datasets.}
    \label{tab:finetune_hyper}
    \begin{tabular}{l|c|c|c|c}
    \hline
        \textbf{Dataset} & \textbf{CIFAR-10} &  \textbf{TinyImageNet} & \textbf{CelebAMask-HQ} & \textbf{WFLW}  \\\hline
        Optimizer & SGD & SDG & SGD  & Adam \\\hline
        lr & 0.1 & 0.1 & 0.01 & 2e-3 \\\hline
        bs & 128 & 128 & 16 & 128\\\hline
        momentum & 0.9 & 0.9 & 0.9 & -  \\\hline
        weight decay & 1e-4 & 1e-4 & 5e-4 & 0\\\hline
        lr decay & step decay at [100, 150] epoch & step decay at [100, 150] epoch & polynomial decay & step decay at [40, 55] epoch \\\hline
        EMA momentum & 0.999 & 0.999 & 0.999 & 0.999 \\\hline
        training time &  200 epoch  &200 epoch & 160k iters & 60 peoch \\ \hline
    \end{tabular}

\end{table}
\begin{table}[H]
    \centering
        \caption{Distillation feature pairs between teacher and students.}
    \label{tab:featurematchs}
    \begin{tabular}{c|l|l}
    \hline
    Dataset & \textbf{CIFAR-10} & \textbf{TinyImageNet}\\\hline
        Teacher Layer & \texttt{mid\_block.resnets.1.conv2} & \texttt{mid\_block.resnets.2.conv3} \\\hline
        \multirow{2}{*}{Student Layer} & R18:\texttt{layer4.1.relu} & R18:\texttt{layer4.1.relu} \\
&MBNv2:\texttt{conv2.activate}&MBNv2:\texttt{conv2.activate}\\
        \hline
    \end{tabular}
        \begin{tabular}{c|l}
    \hline
    Dataset & \textbf{CelebAMAsk-HQ} 
    \\\hline
        Teacher Layer & \texttt{mid\_block.resnets.1.conv2} 
        \\\hline
        \multirow{3}{*}{Student Layer} & R18:\texttt{layer4.1.relu}  \\ &R50:\texttt{layer4.2.relu} \\
        &HRNet18:\texttt{stage4.2.relu}\\
        \hline
    \end{tabular}

\end{table}

\subsection{Landmark Detection}
The pre-trained weights obtained from the distilled face parsing models are utilized to perform face landmark detection. The training of the model is carried out on the WFLW dataset, which comprises 98 annotated key points. An annotated illustration is provided in Figure~\ref{fig:anno_wflf}.
% \begin{wrapfigure}{r}{0.15\textwidth}

The Top-down heatmap-based keypoint estimation technique, as described in~\cite{xiao2018simple}, was implemented using \texttt{mmpose}\footnote{\url{https://github.com/open-mmlab/mmpose}}. Table\ref{tab:finetune_hyper} contains the hyper-parameters used for training the landmark detectors.

% \end{wrapfigure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.15\textwidth]{iccv2023AuthorKit/fig/WFLW.png}
\caption{Illustration for the 98 annotated facial landmarks for WFLW.}
\label{fig:anno_wflf}
\end{figure}




\subsection{Image Classification} 
On TinyImageNet training, we used a $64\times64$ guided diffusion model that was specifically trained with class labels as input conditions. Although unconditional DPMs were used for other tasks, in our case, we included the class label as an input during the distillation process on the TinyImageNet.

In addition, the hyperparameters utilized during the distillation process are presented in Table~\ref{tab:distill_hyper}, while Table~\ref{tab:finetune_hyper} lists the hyperparameters for fine-tuning. Furthermore, Table~\ref{tab:featurematchs} provides a description of the distillation feature pairs.
